BlinkDB: Queries with Bounded Errors and Bounded Response Times on Very Large Data

In this paper, we present BlinkDB, a massively parallel, sampling-based approximate query engine for running ad-hoc, interactive SQL queries on large volumes of data. The key insight that BlinkDB builds on is that one can often make reasonable decisions in the absence of perfect answers. For example, reliably detecting a malfunctioning server using a distributed collection of system logs does not require analyzing every request processed by the system. Based on this insight, BlinkDB allows one to trade-off query accuracy for response time, enabling interactive queries over massive data by running queries on data samples and presenting results annotated with meaningful error bars. To achieve this, BlinkDB uses two key ideas that differentiate it from previous work in this area: (1) an adaptive optimization framework that builds and maintains a set of multi-dimensional, multi-resolution samples from original data over time, and (2) a dynamic sample selection strategy that selects an appropriately sized sample based on a query's accuracy and/or response time requirements. We have built an open-source version of BlinkDB and validated its effectiveness using the well-known TPC-H benchmark as well as a real-world analytic workload derived from Conviva Inc. Our experiments on a 100 node cluster show that BlinkDB can answer a wide range of queries from a real-world query trace on up to 17 TBs of data in less than 2 seconds (over 100\times faster than Hive), within an error of 2 - 10%.

==> Makefile <==
.PHONY: all clean dist print

P = paper

SPELLTEX=$(shell egrep '^\\\input' paper.tex | sed 's/^.*input[^{]*{//' | sed 's/}.*$$/.tex/')

default : $P.pdf

publish : $P.pdf
	scp $P.pdf sameerag@login.eecs.berkeley:~/public_html/blinkdb-draft.pdf

$P.dvi	: $(wildcard *.tex *.bib *.sty *.cls)
	latex  $P < /dev/null || $(RM) $@
	bibtex $P < /dev/null || $(RM) $@
	latex  $P < /dev/null || $(RM) $@
	latex  $P < /dev/null || $(RM) $@

# dvipdf -Tletter $P.dvi $P.pdf
$P.pdf	: $(wildcard *.tex *.bib *.sty *.cls)
	pdflatex  $P < /dev/null || $(RM) $@
	bibtex $P < /dev/null || $(RM) $@
	pdflatex  $P < /dev/null || $(RM) $@
	pdflatex  $P < /dev/null || $(RM) $@
	chmod +x $P.pdf

paper-diff.pdf : $P.pdf # hack to pull in all dependencies of P.pdf
	latexdiff --flatten paper.tex paper-in.tex > paper-diff.tex
	pdflatex paper-diff
	bibtex paper-diff
	pdflatex paper-diff
	pdflatex paper-diff

%.pdf : %.svg
	./svg2pdf $<

%.eps : %.svg
	./svg2eps $<

%.pdf : %.eps
	epstopdf $< -o $@

%.eps : %.ps
	ps2eps -R + -f $<

$P.ps	: $P.dvi
	dvips -t letter $P.dvi -o $P.ps

$P.ps.gz: $P.ps
	$(RM) $P.ps.gz
	gzip -9 < $P.ps > $P.ps.gz

spellcheck:
	for i in $(SPELLTEX); do \
	  echo $$i; \
	  aspell -c --home-dir=. $$i; \
	done

print:	$P.ps

dist:	$P.ps.gz

clean:
	$(RM) $P.log $P.aux $P.bbl $P.blg $P.dvi $P.ps $P.ps.gz texput.log $P.out $P.pdf

camera.pdf: paper.dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 paper.dvi
	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true paper.ps
	cp paper.pdf camera.pdf


==> background.tex <==
 %!TEX root = vldb.tex
%\section{background}\label{background}


==> results.tex <==
 %!TEX root = vldb.tex
\section{Experimental Results}\label{results}
\subsection{Synthetic Workload}
To test our system we rely on synthetic data generated by a tool, with similar characteristics as that of the user access logs from Conviva Inc. Our generator produces data where some fields, for instance zip code, city and state, are closely correlated, while others, for instance the site visited, and session length are loosely correlated. The distribution of most of the rows is derived from data found on the internet about machine, and browser popularity, ISP popularity, and assumptions about the population of different cities. We believe that such synthetic data allows us to test many aspects of our system, in particular, it allows us to test the efficiency of our sample selection strategy, our selectivity in the face of filtering clauses, performance of the overall system, etc. In addition to testing on synthetic data, we also plan on testing our system on real, anonymized data acquired from Conviva Inc, and other sources.

\begin{table}[htdp]
\caption{Fields in Synthetic Data}
\begin{center}
\begin{tabular}{|l|l|l|}
\hline
\bf{Name} & \bf{Type} & \bf{Description} \\
\hline
\texttt{session\_id} & \texttt{int} & Session ID \\
\texttt{session\_start} & \texttt{double} & Start time \\
\texttt{session\_end} & \texttt{double} & End time \\
\texttt{session\_state} & \texttt{int} & HTTP status\\
\texttt{error\_code} & \texttt{int} & Error code, in case of errors\\
\texttt{user\_id} & \texttt{int} & User ID\\
\texttt{country} & \texttt{string} & User country\\
\texttt{city} & \texttt{string} & User city\\
\texttt{state} & \texttt{string} & User state\\
\texttt{zipcode} & \texttt{string} & Zipcode\\
\texttt{content\_id} & \texttt{int} & Content-ID\\
\texttt{ip\_address} & \texttt{string} & IP address\\
\texttt{provider} & \texttt{string} & Provider \\
\texttt{os\_type} & \texttt{string} & Operating System \\
\texttt{os\_version} & \texttt{string} & OS version \\
\texttt{flash\_type} & \texttt{string} & Is Flash present\\
\texttt{flash\_version} & \texttt{string} & Flash Player version\\
\hline
\end{tabular}
\end{center}
\label{default}
\end{table}

In addition to these tables, we use a synthetic workload generator to generate a variety of queries, and use these queries to both test the system, and the effectiveness of our sample selection strategy. Our current queries are based on the kinds of generic queries one would expect to run on data as structured above, and on data from Conviva Inc about the kind of queries they use. We plan on eventually running some of the TPC-H workloads for further testing.

\subsection{Benchmarks}

\begin{figure}[]
\begin{center}
\includegraphics*[width=225px]{figures/ErrorBarsWithTimeForAverage.pdf}
\caption{Variation of error (with a 95\% confidence interval) and query latency with respect to sample sizes for a query that calculates the average session duration: \texttt{select avg(session\_end - session\_start) from syntheticvistordata}}
\label{avg}
\end{center}
\end{figure}

\begin{figure}[]
\begin{center}
\includegraphics*[width=225px]{figures/count.pdf}
\caption{Variation of error (with a 95\% confidence interval) and query latency with respect to sample sizes for a query that calculates the number of entries in the database: \texttt{select count(*) from syntheticvistordata}}
\label{count}
\end{center}
\end{figure}

We evaluated \system~by storing 9GB of our synthetic workload data in
HDFS running across 3 Amazon EC2 large instances (7.5GB RAM, 4 EC2
Compute Units and high I/O performance). In order to compare the
tradeoffs between sample size, error bars and query latency, we then
created sixteen samples of varying sizes ranging from 2KB to 64MB in
multiples of two. Figure~\ref{avg} plots the query latency and error
bars at 95\% confidence interval as a function of sample sizes for the
\texttt{average} operator.  For the purpose of this experiment, all
the input tables were cached in memory as an RDD and the the query
computed the average of the user session duration
(\texttt{session\_end - session\_start}). Figure~\ref{count} similarly
plots the count query latency and error bars at 95\% confidence
interval as a function of sample sizes for the \texttt{count}
operator.  This query computed the number of entries in the table and
also operated on in-memory samples.

To evaluate the efficiency of our statistical method we ran a few
benchmarks outside of the cluster. These benchmarks were run on data
drawn from a gamma distribution, from which we drew a limited size
sample. In the graph shown in Figure~\ref{blb-perf-fig1} we evaluated
the performance of BLB in accurately computing the variance of the
k-means operator when applied over a fixed size sample. We evaluated
the quality by first computing the variance of k-means over a large
set of samples, of the same size, drawn from the underlying
distribution, on which we ran the k-means algorithm. We then compared
the variance returned by bag of little bootstraps, against this
variance. As the graph shows, the error in our variance calculation
decreases rapidly, and BLB is in face an effective method for
calculating the variance in the distribution of a complex function.

To evaluate the quality of BLB vs a more traditional analytical approach, we ran a set of experiments comparing standard error of mean, with both BLB and traditional bootstrap. All the methods were used to calculate variance of the mean, for a sample drawn from the gamma distribution. As can be seen in Figure~\ref{blb-perf-fig2}, the performance of all three methods is similar, and BLB does in fact behave in a manner very similar to traditional closed form approaches. We would have expected BLB to perform slightly better, given that bootstrap should in theory show faster convergence than other methods, however for variance, bootstrap can perform no better than the traditional closed form version.

\begin{figure}[]
\begin{center}
\includegraphics*[width=225px]{figures/kmeans.pdf}
\caption{Evaluating BLB performance in predicting variance in K-Means}
\label{blb-perf-fig1}
\end{center}
\end{figure}

\begin{figure}[]
\begin{center}
\includegraphics*[width=225px]{figures/AlgorithmComparison.pdf}
\caption{Evaluating BLB vs bootstrap vs standard error of mean for computing variance of mean}
\label{blb-perf-fig2}
\end{center}
\end{figure}


%{\color{red}0. Synthetic workload. 1.We created samples from 2KB to 64MB in size and evaluated the variation of sample size with query latency and error bars. 2. Comparison of %Bootstrap and Closed form error 3. Micro-benchmarks on BLB. 4. End-to-end Query latency.}

